Subcubic Equivalences Between Graph Centrality Measures and Complementary Problems

Despite persistent efforts, there is no known technique for obtaining unconditional super-linear lower bounds for the computational complexity of the problems in P. Vassilevska Williams and Williams introduce a fruitful approach to advance a better understanding of the computational complexity of the problems in P. In particular, they consider All Pairs Shortest Paths (APSP) and other fundamental problems such as checking whether a matrix defines a metric, verifying the correctness of a matrix product, and detecting a negative triangle in a graph. Abboud, Grandoni, and Vassilevska Williams study well-known graph centrality problems such as Radius, Median, etc., and make a connection between their computational complexity to that of two fundamental problems, namely APSP and Diameter. They show any algorithm with subcubic running time for these centrality problems, implies a subcubic algorithm for either APSP or Diameter. In this paper, we define vertex versions for these centrality problems and based on that we introduce new complementary problems. The main open problem of Abboud et al. is whether or not APSP and Diameter are equivalent under subcubic reduction. One of the results of this paper is APSP and CoDiameter, which is the complementary version of Diameter, are equivalent. Moreover, for some of the problems in this set, we show that they are equivalent to their complementary versions. Considering the slight difference between a problem and its complementary version, these equivalences give us the impression that every problem has such a property, and thus APSP and Diameter are equivalent. This paper is a step forward in showing a subcubic equivalence between APSP and Diameter, and we hope that the approach introduced in our paper can be helpful to make this breakthrough happen.

==> approx.tex <==
\section{The Approximation Version of Problems}
Here, we give new lower bound on the hardness of approximation for \Radius{}, \CoRadius{}, \CODiameter{}.
We show that a $4/3-\epsilon$ approximation algorithm for \Radius{} in time $O(n^{\omega-\delta})$ (for a $\delta > 0$) would violate a widely believed conjecture about the \kclique{} problem. In addition, a combinatorial $4/3-\epsilon$ approximation algorithm for \Radius{} in time $O(n^{3-\delta})$ (for $\delta > 0$) would violate another conjecture about the \kclique{} problem.
We use the same method to prove similar results for $\mathsf{(4/3-\epsilon)-gap\, CoRadius}$ and $\mathsf{(4/3-\epsilon)-gap\, CoDiameter}$.

Our lower bounds are based on a conjecture about \kclique{}. Before we present our reductions, we should briefly discuss the conjectures and the \kclique{} problem itself. \textsf{k-Clique} is a fundamental graph problem that asks weather an undirected, unweighted graph contains a clique of size $k$. This problem is the parameterized version of the \textsf{Max-Clique} problem, which is NP-complete \cite{Kar72}.
In parameterized complexity \kclique{} is W[1]-complete.
\kclique{} can be solved using fast matrix multiplication in time $O(n^{\omega k/3})$ time \cite{3clique}, for $k=0\,(mod\: 3)$. For $k=1,2\,(mod\: 3)$, the running time is slightly more \cite{EG04}. In the case of combinatorial algorithm, the fastest algorithm runs in $O(n^k/\log^k n)$ time \cite{Vas09}. 

The lack of better algorithms leads to two conjectures below in fields of graph algorithms and parameterized complexity \cite{valiant, Woe04, Aut84}.
Furthermore, refuting the second conjecture implies a faster exact algorithm for $\mathsf{MAX-CUT}$~\cite{Wil05, Woe04}.

\begin{conjecture}[Combinatorial \kclique{}]\label{combkcli}
Let $0\leq C\leq 3$ be the smallest number such that $\mathsf{3k-Clique}$ can be solved combinatorially in $O(n^{Ck})$ time by any algorithm, for any (large enough) constant $k\in \mathbb{N}$. The conjecture is that $C=3$.
\end{conjecture}

\begin{conjecture}[\kclique{}]\label{kcil}
Let $0\leq F\leq \omega$ be the smallest number such that $\mathsf{3k-Clique}$ can be solved in $O(n^{Fk})$ time by any algorithm, for any (large enough) constant $k\in \mathbb{N}$. The conjecture is that $F=\omega$.
\end{conjecture}

\kclique{} has been reduced to $\mathsf{3-Clique}$ and BMM~\cite{3clique}, \textsf{CNF Parsing}, \textsf{RNA Folding} and \textsf{Dyck Language Edit Distance}~\cite{valiant}, max weight rectangle problem~\cite{maxrect}, word break~\cite{wordbreak}, and used to prove the hardness of improving Viterbi’s algorithm.
%
%Ne{\v{s}}et{\v{r}}il and Poljak reduce \kclique{} to $\mathsf{3-Clique}$ and BMM~\cite{3clique}.
%Aboud, Buckers and V. Williams reduce \kclique{} to three problems of \textsf{CNF Parsing}, \textsf{RNA Folding} and \textsf{Dyck Language Edit Distance}~\cite{valiant}.
%Backurs and Tzamos study the hardness of improving Viterbi’s algorithm using a reduction from \kclique{}~\cite{viterbi}.
%Backurs, Dikkala, and Tzamos reduced \kclique{} to the max weight rectangle problem~\cite{maxrect}.
%Bringmann, Grønlund, and Larsen reduced \kclique{} Word Break~\cite{wordbreak}.
Given that most of these results are very recent, we expect that the family of \kclique{}--hard problems will grow in future. However, our work is the first use of \kclique{} to proving the inapproximability of a problem.


Now, we are ready to present our reductions. We can reduce \kclique{} to our problem directly, or by using one of the \kclique{}--hard problems mentioned above as an intermediate problem. For that matter, we reduce from the $\mathsf{3-Clique}$ problem. The reduction to $\mathsf{(4/3-\epsilon)-\Radius}$ uses some ideas from a reduction from \NEG{} to \Radius{}~\cite{soda}; however, that reduction is incapable of producing any gaps. We use additional ideas and carefully adjusted edge weights to produce a gap as large as possible. We construct an undirected graph in our reduction, thus our lower bound applies to both directed and undirected versions of \Radius{}.
%
Formally, our reduction from $\mathsf{3-Clique}$ to $\mathsf{(4/3-\epsilon)-Radius}$ proves the following lemma.

\begin{lemma}
\label{3cl2rad}
Given an $T(n)$ time algorithm for $\mathsf{(4/3-\epsilon)-Radius}$, where $T(n)$ is polynomial in $n$, there exists an $O(T(n) + n^2)$ time algorithm for $\mathsf{3-Clique}$. Moreover, the reduction is combinatorial.
\end{lemma}

The proof of Lemma \ref{3cl2rad} is in Appendix \ref{omittedProofs}.
The following theorem follows directly from Lemma \ref{3cl2rad}.

\begin{theorem}$\mathsf{3-Clique}\leq_{n^\omega}\mathsf{(4/3-\epsilon)-\Radius}$
\end{theorem}

Similar to Lemma \ref{radToCorad}, we can add two vertices $z$ and $z'$ to graph $G$. We set $w(z,z')=8$ and $w(z, h)=4$ for $h\in V(G')\backslash \{z\}$ and $w(z', h)=4$ for $h\in V(G')\backslash \{z'\}$. A similar argument proves the next theorem.
%A similar argument to Lemma \ref{radToCorad} proves the next theorem.

\begin{theorem}
$\mathsf{3-Clique}\leq_{n^\omega}\mathsf{(4/3-\epsilon)-gap\, CoRadius}$
\end{theorem}

Using an observation similar to Observation \ref{obvious}, our reduction also works for $\mathsf{(4/3-\epsilon)-gap}$ $\mathsf{CoDiameter}$.

\begin{corollary}
$\mathsf{3-Clique}\leq_{n^\omega}\mathsf{(4/3-\epsilon)-gap\, CoDiameter}$
\end{corollary}

	


==> omittedProofs.tex <==
%\section{Omitted Proofs} \label{omittedProofs}

\begin{proofof}{Lemma \ref{3cl2rad}}
Given a graph $G$, we construct a undirected, weighted graph $G'$ such that, to solve the triangle ($\mathsf{3-Clique}$) problem for $G$, we can solve \Radius{} for $G'$.
For an instance $G$ with $n$ vertices, we construct a undirected, weighted graph $G'$ with $4n+2$ vertices. More precisely, $V(G')$ is consisted of four parts $A$, $B$, $C$, and $A'$, each containing $n$ nodes, plus two additional vertices, x and y. For every vertex $v\in V(G)$, we put vertices $v_{A}$, $v_{B}$, $v_{C}$, and $v_{A'}$ in parts $A$, $B$, $C$, and $A'$, respectively. We complete the construction of the graph with the following edge weight assignments. Note that $G'$ is a complete graph and $w(u,v)$ is the weight of edge $(u,v)\in G'$.
\begin{itemize}
\item
$w(u_A, v_B), w(u_B, v_C), w(u_C, v_{A'}) =
\begin{cases}
2 & (u,v)\in E(G), \\
4 & \text{otherwise,}
\end{cases}
$
\item
$w(u_A, v_C) = 6\text{ for all }u,v\in V(G),$
\item
$w(u_A, v_{A'}) = 6\text{ for all }u,v\in V(G)\text{ where }u\neq v,$
\item
$w(x, u_A) = 3\text{ for all }u\in V(G),$
\item
$w(x,y)=3,$
\item
$\text{other edge weightes} = 8.$
\end{itemize}
%
Due to the construction of $G'$, the eccentricity of all $b_v$'s, $c_v$'s, $a'_v$'s, $x$, and $y$ is at least $8$. The eccentricity of $a_v$ is $6$ if $v$ is in a triangle in $G$, and $8$ otherwise. Therefore, the radius is $6$ if $G$ has a triangle, and $8$ otherwise. Hence, any $4/3-\epsilon$ approximation of \Radius{} can solve the triangle problem or $\mathsf{3-Clique}$. The construction of $G'$ takes time $O(n^2)$. Therefore, any $T(n)$ time algorithm for $\mathsf{(4/3 - \epsilon) - Radius}$, where $T(n)$ is polynomial in $n$, can be used to solving $\mathsf{3-Clique}$ in time $O(T(n) + n^2)$. Due to the construction of $G'$, the reduction is combinatorial.
\end{proofof}



==> our-results.tex <==
There are our results. :)
